Neural Normalized Min-Sum Message-Passing vs. Viterbi Decoding for the CCSDS Line Product Code

The Consultative Committee for Space Data Systems (CCSDS) 141.11-O-1 Line Product Code (LPC) provides a rare opportunity to compare maximum-likelihood decoding and message passing. The LPC considered in this paper is intended to serve as the inner code in conjunction with a (255,239) Reed Solomon (RS) code whose symbols are bytes of data. This paper represents the 141.11-O-1 LPC as a bipartite graph and uses that graph to formulate both maximum likelihood (ML) and message passing algorithms. ML decoding must, of course, have the best frame error rate (FER) performance. However, a fixed point implementation of a Neural-Normalized MinSum (N-NMS) message passing decoder closely approaches ML performance with a significantly lower complexity.

==> cn.tex <==
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
      & \begin{tabular}[c]{@{}c@{}}Number of VNs\\ in sub-block 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}Number of VNs\\ in sub-block 2\end{tabular} \\ \hline
$c_0$ & 4                                                                      & 0                                                                      \\ \hline
$c_1$ & 5                                                                      & 0                                                                      \\ \hline
$c_2$ & 1                                                                      & 4                                                                      \\ \hline
$c_3$ & 1                                                                      & 4                                                                      \\ \hline
$c_4$ & 2                                                                      & 2                                                                      \\ \hline
$c_5$ & 2                                                                      & 3                                                                      \\ \hline
$c_6$ & 2                                                                      & 3                                                                      \\ \hline
$c_7$ & 2                                                                      & 3                                                                      \\ \hline
\end{tabular}
\end{center}

